Who's Asking? Audience-Conditioned Privatization

The abundance of user-generated conversational data makes the question of how to responsibly derive insights from confidential data without putting the individuals in it at risk ever more important. However, the majority of existing differentially private (DP) synthetic text generation (SDG) and anonymization approaches ignore the context of the data's downstream usage, which results in loss of important information. DP-SDG provides the same guarantee regardless of the recipient, and anonymization relies on predefined attribute categories. They both ignore the observation that an attribute that is harmless to one audience can be sensitive to another, and each audience typically needs only some attributes preserved. We propose Ext-Classify-Priv, a framework that (1) extracts the information types present in a corpus, (2) classifies which of them are private for a given audience following contextual integrity, and (3) protects only those attributes, using either anonymization or SDG with Feature-DP approaches. On Reddit data with 3 audiences, our audience-specific releases are more faithful than a single audience-agnostic release for every audience. On bioRxiv data, our SDG method improves MAUVE from 0.097 to 0.420 at epsilon=1 and on the proprietary real estate data, our anonymization method improves MAUVE from 0.698 to 0.959 over the best baselines.

==> diagram_fairness.tex <==
% =====================================================================
%  Fairness evaluation (performance discrepancy by subgroup)
%
%  Self-contained figure file: \input{fairness_eval_figure} in the paper body.
%  Preamble requirements:
%     \usepackage{tikz}
%     \usetikzlibrary{arrows.meta,fit,positioning,decorations.pathreplacing,calc,backgrounds}
%     \usepackage{amssymb,pifont}
%  The definitions below use \providecommand / \colorlet / \tikzset, so
%  inputting both evaluation figures (or the pipeline figures) is safe.
%  For a two-column paper spanning both columns, change figure -> figure*
%  and \columnwidth -> \textwidth.
% =====================================================================

% ---------- shared definitions (put once, e.g. in the preamble) ----------
\colorlet{privcol}{red!70}
\colorlet{mechcol}{blue!60}
\colorlet{pubcol}{green!55!black}

% inline span highlights inside document cards
\providecommand{\sneu}[1]{{\setlength{\fboxsep}{0.7pt}\colorbox{black!11}{#1}}}%   extracted, unclassified
\providecommand{\spub}[1]{{\setlength{\fboxsep}{0.7pt}\colorbox{black!11}{#1}}}%   public, kept as-is
\providecommand{\spriv}[1]{{\setlength{\fboxsep}{0.7pt}\colorbox{privcol!22}{#1}}}% private
\providecommand{\ssyn}[1]{{\setlength{\fboxsep}{0.7pt}\colorbox{pubcol!32}{\textcolor{pubcol!45!black}{#1}}}}% synthesized
\providecommand{\spk}[1]{\textbf{#1:}\,}%                                            speaker tag

\tikzset{
  % document cards
  doccard/.style={draw=privcol!80,fill=privcol!4,rounded corners=2pt,line width=0.6pt,
                  align=left,font=\scriptsize,inner sep=3pt,minimum height=0.78cm,
                  execute at begin node={\hyphenpenalty=10000\exhyphenpenalty=10000}},
  relcard/.style={doccard,draw=pubcol!85,fill=pubcol!5},
  % table cells: <kind>h = header, <kind>c = value cell
  tcell/.style={draw=white,line width=0.8pt,inner sep=0pt,font=\scriptsize},
  neuh/.style={tcell,fill=black!22,text=black!80},
  neuc/.style={tcell,fill=black!7,text=black!80},
  pubh/.style={tcell,fill=pubcol!60,text=white},
  pubc/.style={tcell,fill=pubcol!14,text=black!80},
  privh/.style={tcell,fill=privcol!65,text=white},
  privc/.style={tcell,fill=privcol!14,text=black!80},
  synh/.style={tcell,fill=pubcol!60,text=white},
  sync/.style={tcell,fill=pubcol!30,text=pubcol!40!black,font=\scriptsize\itshape},
  % boxes
  grp/.style={draw=black!35,dashed,rounded corners=3pt,inner sep=4pt},
  stepbox/.style={draw=black!45,fill=black!3,rounded corners=3pt,line width=0.8pt,
                  text=black!75,align=center,font=\footnotesize},
  mech/.style={draw=mechcol,fill=mechcol!8,rounded corners=3pt,line width=0.9pt,
               text=mechcol!80!black,align=center,font=\footnotesize},
  submech/.style={draw=mechcol!70,fill=white,rounded corners=2pt,line width=0.6pt,
                  text=mechcol!80!black,align=center,font=\scriptsize,inner sep=2.5pt},
  % arrows
  inar/.style={->,draw=privcol!70,line width=0.7pt},
  outar/.style={->,draw=pubcol!70,line width=0.8pt},
  neuar/.style={->,draw=black!45,line width=0.7pt},
  mechar/.style={->,draw=mechcol!70,line width=0.7pt},
  % text
  lbl/.style={font=\scriptsize\itshape},
  brace/.style={decorate,decoration={brace,amplitude=4pt},draw=black!50,line width=0.6pt},
}

\tikzset{
  evalbox/.style={draw=black!45,fill=black!3,rounded corners=3pt,line width=0.7pt,
              text=black!75,align=center,font=\scriptsize,inner sep=3pt},
  tgtcol/.style={draw=black!75,dashed,line width=0.8pt,inner sep=0pt},
}

\begin{figure}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}[>={Stealth[length=2mm]},font=\small]

%% training sources -> downstream models
\node[doccard,text width=1.6cm,align=center,minimum height=0.6cm] (s1) at (0,2.9) {real $\mathcal{D}$};
\node[relcard,text width=1.6cm,align=center,minimum height=0.6cm] (s2) at (0,2.0) {high $\varepsilon$};
\node[relcard,text width=1.6cm,align=center,minimum height=0.6cm,fill=pubcol!2,draw=pubcol!55] (s3) at (0,1.1) {low $\varepsilon$};

\node[evalbox,text width=1.9cm,minimum height=2.4cm] (ev) at (3.2,2.0)
  {train, then\\ evaluate on\\ real test data\\ \emph{per subgroup}};
\foreach \s in {1,2,3} \draw[neuar] (s\s.east) -- (ev.west |- s\s);

%% schematic grouped bar chart
\def\bx{5.0}\def\by{0.7}
\draw[->,black!55,line width=0.6pt] (\bx,\by) -- (\bx,3.65)
  node[above,font=\tiny,text=black!65] {performance};
\draw[black!55,line width=0.6pt] (\bx,\by) -- (10.6,\by);
\foreach \g/\c/\hr/\hh/\hl in {1/6.2/2.40/2.30/2.15, 2/8.0/2.35/2.20/1.90, 3/9.8/2.30/1.95/1.05}{
  \fill[privcol!55] (\c-0.62,\by) rectangle ++(0.38,\hr);
  \fill[pubcol!80]  (\c-0.19,\by) rectangle ++(0.38,\hh);
  \fill[pubcol!30]  (\c+0.24,\by) rectangle ++(0.38,\hl);
  \node[font=\scriptsize,text=black!70,anchor=north] at (\c,\by) {$g_{\g}$};
}
\draw[densely dotted,black!50] (9.8-0.62,{\by+2.30}) -- (10.55,{\by+2.30});
\draw[densely dotted,black!50] (9.8+0.62,{\by+1.05}) -- (10.55,{\by+1.05});
\draw[<->,black!70,line width=0.6pt] (10.5,{\by+2.30}) -- (10.5,{\by+1.05})
  node[midway,right,font=\scriptsize\itshape,align=left,text=privcol!80!black]
  {gap in performance\\ increased};
\draw[neuar] (ev.east) -- (\bx-0.1,2.0);

%% legend
\foreach \i/\col/\txt in {0/privcol!55/real,1/pubcol!80/{high $\varepsilon$},2/pubcol!30/{low $\varepsilon$}}{
  \fill[\col] ({5.9+1.45*\i},3.55) rectangle ++(0.25,0.18);
  \node[font=\tiny,anchor=west,text=black!70] at ({6.2+1.45*\i},3.64) {\txt};
}

\end{tikzpicture}}
\caption{\textbf{Fairness evaluation via performance discrepancy across subgroups.} The same
downstream model is trained on the real data $\mathcal{D}$ and on synthetic data generated at a high
and at a low privacy budget $\varepsilon$. Each model is evaluated on held-out real test data, and
its performance is reported separately for each demographic subgroup $g_1,g_2,g_3$. Some loss in
performance is expected as $\varepsilon$ decreases; a fairness violation occurs when this loss is
uneven across subgroups, i.e., when the gap in performance between subgroups widens significantly as
privacy tightens (here, for $g_3$). Bar heights are illustrative.}
\label{fig:eval-fairness}
\end{figure}

==> diagram_privacy.tex <==
% =====================================================================
%  Privacy evaluation by attribute inference
%
%  Self-contained figure file: \input{privacy_eval_figure} in the paper body.
%  Preamble requirements:
%     \usepackage{tikz}
%     \usetikzlibrary{arrows.meta,fit,positioning,decorations.pathreplacing,calc,backgrounds}
%     \usepackage{amssymb,pifont}
%  The definitions below use \providecommand / \colorlet / \tikzset, so
%  inputting both evaluation figures (or the pipeline figures) is safe.
%  For a two-column paper spanning both columns, change figure -> figure*
%  and \columnwidth -> \textwidth.
% =====================================================================

% ---------- shared definitions (put once, e.g. in the preamble) ----------
\colorlet{privcol}{red!70}
\colorlet{mechcol}{blue!60}
\colorlet{pubcol}{green!55!black}

% inline span highlights inside document cards
\providecommand{\sneu}[1]{{\setlength{\fboxsep}{0.7pt}\colorbox{black!11}{#1}}}%   extracted, unclassified
\providecommand{\spub}[1]{{\setlength{\fboxsep}{0.7pt}\colorbox{black!11}{#1}}}%   public, kept as-is
\providecommand{\spriv}[1]{{\setlength{\fboxsep}{0.7pt}\colorbox{privcol!22}{#1}}}% private
\providecommand{\ssyn}[1]{{\setlength{\fboxsep}{0.7pt}\colorbox{pubcol!32}{\textcolor{pubcol!45!black}{#1}}}}% synthesized
\providecommand{\spk}[1]{\textbf{#1:}\,}%                                            speaker tag

\tikzset{
  % document cards
  doccard/.style={draw=privcol!80,fill=privcol!4,rounded corners=2pt,line width=0.6pt,
                  align=left,font=\scriptsize,inner sep=3pt,minimum height=0.78cm,
                  execute at begin node={\hyphenpenalty=10000\exhyphenpenalty=10000}},
  relcard/.style={doccard,draw=pubcol!85,fill=pubcol!5},
  % table cells: <kind>h = header, <kind>c = value cell
  tcell/.style={draw=white,line width=0.8pt,inner sep=0pt,font=\scriptsize},
  neuh/.style={tcell,fill=black!22,text=black!80},
  neuc/.style={tcell,fill=black!7,text=black!80},
  pubh/.style={tcell,fill=pubcol!60,text=white},
  pubc/.style={tcell,fill=pubcol!14,text=black!80},
  privh/.style={tcell,fill=privcol!65,text=white},
  privc/.style={tcell,fill=privcol!14,text=black!80},
  synh/.style={tcell,fill=pubcol!60,text=white},
  sync/.style={tcell,fill=pubcol!30,text=pubcol!40!black,font=\scriptsize\itshape},
  % boxes
  grp/.style={draw=black!35,dashed,rounded corners=3pt,inner sep=4pt},
  stepbox/.style={draw=black!45,fill=black!3,rounded corners=3pt,line width=0.8pt,
                  text=black!75,align=center,font=\footnotesize},
  mech/.style={draw=mechcol,fill=mechcol!8,rounded corners=3pt,line width=0.9pt,
               text=mechcol!80!black,align=center,font=\footnotesize},
  submech/.style={draw=mechcol!70,fill=white,rounded corners=2pt,line width=0.6pt,
                  text=mechcol!80!black,align=center,font=\scriptsize,inner sep=2.5pt},
  % arrows
  inar/.style={->,draw=privcol!70,line width=0.7pt},
  outar/.style={->,draw=pubcol!70,line width=0.8pt},
  neuar/.style={->,draw=black!45,line width=0.7pt},
  mechar/.style={->,draw=mechcol!70,line width=0.7pt},
  % text
  lbl/.style={font=\scriptsize\itshape},
  brace/.style={decorate,decoration={brace,amplitude=4pt},draw=black!50,line width=0.6pt},
}

\tikzset{
  evalbox/.style={draw=black!45,fill=black!3,rounded corners=3pt,line width=0.7pt,
              text=black!75,align=center,font=\scriptsize,inner sep=3pt},
  tgtcol/.style={draw=black!75,dashed,line width=0.8pt,inner sep=0pt},
}

% a small stack of text documents: #1 name, #2 position, #3 card style, #4 text
\providecommand{\docstack}[4]{%
  \node[#3,text width=2.5cm,font=\tiny,minimum height=0.9cm] (#1) at #2 {#4};
  \begin{scope}[on background layer]
    \node[#3,minimum width=2.5cm+6pt,minimum height=0.9cm,font=\tiny,anchor=center]
      at ([xshift=4pt,yshift=4pt]#1.center) {};
    \node[#3,minimum width=2.5cm+6pt,minimum height=0.9cm,font=\tiny,anchor=center]
      at ([xshift=2pt,yshift=2pt]#1.center) {};
  \end{scope}%
}

\begin{figure}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}[>={Stealth[length=2mm]},font=\small]
\def\rh{0.42}
% column centres / widths: two known (public) columns, two inferred (private) columns
\def\ca{2.725}\def\cb{3.775}\def\cc{4.95}\def\cd{6.25}
\def\wn{1.05}\def\wp{1.3}
\newcommand{\ok}{\,\textcolor{privcol}{\ding{51}}}
\newcommand{\no}{\,\textcolor{pubcol}{\ding{55}}}

%% ======================= (a) synthetic data =======================
% synthetic text -> table (training)
\docstack{Dh}{(0,1.1)}{relcard,minimum height=0.9cm}
  {\spk{Buyer}Up to \$450k, 20\% down; moving for a new job, just us two.}
\node[font=\tiny\itshape,text=pubcol!85!black,anchor=south] at ([yshift=4pt]Dh.north) {$\hat{\mathcal{D}}$ (synthetic text)};
\foreach \c/\w/\name in {\ca/\wn/budget,\cb/\wn/down,\cc/\wp/reason,\cd/\wp/househ.}
  \node[pubh,minimum width=\w cm,minimum height=\rh cm,font=\tiny] at (\c,1.73) {\name};
\foreach \y/\va/\vb/\vc/\vd in
   {1.31/{\$450k}/{20\%}/new job/couple, 0.89/{\$620k}/{\$60k}/retired/{+ 2 kids},
    0.47/{\$380k}/{$\varnothing$}/divorce/single}{
  \node[pubc,minimum width=\wn cm,minimum height=\rh cm,font=\tiny] at (\ca,\y) {\va};
  \node[pubc,minimum width=\wn cm,minimum height=\rh cm,font=\tiny] at (\cb,\y) {\vb};
  \node[pubc,minimum width=\wp cm,minimum height=\rh cm,font=\tiny] at (\cc,\y) {\vc};
  \node[pubc,minimum width=\wp cm,minimum height=\rh cm,font=\tiny] at (\cd,\y) {\vd};
}
\node[minimum width=4.7cm,minimum height={4*\rh cm},inner sep=0pt] (Th) at (4.55,1.1) {};
\draw[neuar] (Dh.east) -- node[above,font=\scriptsize] {$f_S$} (Th.west);

% real held-out text -> table: public columns known, private columns inferred
\docstack{Dt}{(0,-1.1)}{doccard,minimum height=0.9cm}
  {\spk{Buyer}About \$395k, 15\% down; since the divorce it's me and the kids.}
\node[font=\tiny\itshape,text=privcol!85!black,anchor=north] at ([yshift=-1pt]Dt.south) {$\mathcal{D}_{\mathrm{test}}$ (real text)};
\foreach \c/\w/\name/\st in {\ca/\wn/budget/pub,\cb/\wn/down/pub,\cc/\wp/reason/priv,\cd/\wp/househ./priv}
  \node[\st h,minimum width=\w cm,minimum height=\rh cm,font=\tiny] at (\c,-0.47) {\name};
\foreach \y/\va/\vb/\vc/\vd in
   {-0.89/{\$395k}/{15\%}/{divorce\ok}/{+ 2 kids\ok},
    -1.31/{\$700k}/{25\%}/{retired\no}/{+ 2 kids\no},
    -1.73/{\$410k}/{10\%}/{new job\no}/{couple\no}}{
  \node[pubc,minimum width=\wn cm,minimum height=\rh cm,font=\tiny] at (\ca,\y) {\va};
  \node[pubc,minimum width=\wn cm,minimum height=\rh cm,font=\tiny] at (\cb,\y) {\vb};
  \node[privc,minimum width=\wp cm,minimum height=\rh cm,font=\tiny\itshape] at (\cc,\y) {\vc};
  \node[privc,minimum width=\wp cm,minimum height=\rh cm,font=\tiny\itshape] at (\cd,\y) {\vd};
}
\node[tgtcol,minimum width={2*\wp cm},minimum height={4*\rh cm}] (inf) at ({(\cc+\cd)/2},-1.1) {};
\node[font=\tiny\itshape,text=privcol!80!black,anchor=south] at (inf.north) {inferred};
\node[minimum width=4.7cm,minimum height={4*\rh cm},inner sep=0pt] (Tt) at (4.55,-1.1) {};
\draw[inar] (Dt.east) -- node[above,font=\scriptsize,text=black] {$f_S$} (Tt.west);

% classifier: trained on the synthetic table, fills in the private columns
\def\xg{8.45}
\node[evalbox,font=\footnotesize,minimum width=1.3cm,minimum height=0.9cm] (g) at (\xg,0) {classifier};
\draw[neuar] (Th.east) -| node[pos=0.25,above,font=\scriptsize\itshape,text=black!60] {train} (g.north);
\draw[neuar] (g.south) |- node[pos=0.75,below,font=\scriptsize\itshape,text=black!60] {infer} (inf.east);

%% ======================= (b) anonymization =======================
\def\yb{-3.75}\def\xp{9.8}
\docstack{Da}{(0,\yb)}{relcard,minimum height=0.9cm}
  {\spk{Buyer}Up to \$450k with 20\% down, and we're ready to move soon.}
\node[font=\tiny\itshape,text=pubcol!85!black,anchor=north] at ([yshift=-1pt]Da.south) {$\hat{\mathcal{D}}$ (anonymized text)};

\node[evalbox,font=\footnotesize,minimum width=1.3cm,minimum height=0.9cm] (llm) at (\xg,\yb) {LLM};
\draw[neuar] (Da.east) -- node[above,font=\scriptsize\itshape,text=black!60]
  {``Infer the buyer's move reason and household.''} (llm.west);

\foreach \k/\name in {0/reason,1/househ.}
  \node[privh,minimum width=\wp cm,minimum height=\rh cm,font=\tiny] at ({\xp+(\k+0.5)*\wp},\yb+0.63) {\name};
\foreach \y/\vc/\vd in {0.21/{new job\no}/{couple\no}, -0.21/{divorce\ok}/{+ 2 kids\ok}, -0.63/{retired\no}/{single\no}}{
  \node[privc,minimum width=\wp cm,minimum height=\rh cm,font=\tiny\itshape] at ({\xp+0.5*\wp},\yb+\y) {\vc};
  \node[privc,minimum width=\wp cm,minimum height=\rh cm,font=\tiny\itshape] at ({\xp+1.5*\wp},\yb+\y) {\vd};
}
\node[tgtcol,minimum width={2*\wp cm},minimum height={4*\rh cm}] (infb) at ({\xp+\wp},\yb) {};
\node[font=\tiny\itshape,text=privcol!80!black,anchor=north] at (infb.south) {inferred};
\draw[neuar] (llm.east) -- (infb.west);

%% panel labels, separator, readout
\draw[black!22,dashed] (-1.6,-2.55) -- (12.5,-2.55);
\node[font=\footnotesize\bfseries,text=black!65,anchor=north west] at (-1.6,2.95) {(a) synthetic data};
\node[font=\footnotesize\bfseries,text=black!65,anchor=north west] at (-1.6,-2.65) {(b) anonymization};
\node[font=\scriptsize,align=center] at (11.1,-0.9)
  {attack accuracy\\[1pt] \textcolor{pubcol!85!black}{lower $\Rightarrow$ more private}};

\end{tikzpicture}}
\caption{\textbf{Privacy evaluation via attribute inference.} We measure how well an
adversary can recover the private attributes $S_{\mathrm{priv}}$ of real records from the released data.
\textbf{(a)} Synthetic data: the schema extractor $f_S$ is applied both to the synthetic texts
$\hat{\mathcal{D}}$ and to a held-out split of real texts $\mathcal{D}_{\mathrm{test}}$. A classifier
is trained on the synthetic table to predict the private attributes (here, reason for moving and
household) from the public ones (budget and down payment), and is then used to infer the private
attributes of each real held-out record from its public attributes.
\textbf{(b)} Anonymization: no table is released, so an LLM is prompted to infer the removed private
attributes directly from each anonymized text.
In both cases, the inferences are scored against the true values extracted from the original texts
(\textcolor{privcol}{\ding{51}} correct, \textcolor{pubcol}{\ding{55}} incorrect); lower attack accuracy
indicates stronger privacy protection.}
\label{fig:eval-privacy}
\end{figure}

==> exact_tables.tex <==
\begin{table*}[t]
\centering
\small
\caption{Exact values behind Figure~\ref{fig:spider_audiences} (Reddit, one block per audience). Acc is the accuracy of a RoBERTa classifier trained on the released text and tested on real data; $|\Delta|$ is its accuracy gap between female and male authors. Raw values in natural units ($\uparrow$ higher is better, $\downarrow$ lower is better); best value per family and panel in bold (ties all bold). Len-W is the Wasserstein distance between text-length distributions. Leak is the attack success on the audience's private attributes: attribute-inference advantage over the majority baseline (clipped at 0, averaged over private attributes) for SDG, and LLM fuzzy reconstruction rate (averaged over private attributes) for anonymization. The figures plot MAUVE, $1/(1+\mathrm{KL})$, $1-\mathrm{TV}$, $1/(1+\text{Len-W}/100)$, Acc, $1-|\Delta|$ and $1-\text{Leak}$ on a fixed $[0,1]$ scale.}
\label{tab:spider_audiences}
\begin{tabular}{llrrrrrrr}
\toprule
 & Method & MAUVE$\uparrow$ & KL$\downarrow$ & TV$\downarrow$ & Len-W$\downarrow$ & Acc$\uparrow$ & $|\Delta|\downarrow$ & Leak$\downarrow$ \\
\midrule
\multicolumn{9}{l}{\textit{External Analytics}} \\
SDG ($\varepsilon=1$) & SDG-CI & \textbf{0.479} & \textbf{0.791} & \textbf{0.422} & \textbf{12.7} & \textbf{0.546} & 0.038 & 0.004 \\
 & MAPLE & 0.350 & 1.178 & 0.535 & 36.5 & 0.527 & \textbf{0.003} & \textbf{0.000} \\
 & Aug-PE & 0.027 & 10.557 & 0.814 & 45.1 & 0.522 & 0.084 & 0.001 \\
\cmidrule(l){2-9}
Anon. & AN-CI & \textbf{1.000} & \textbf{0.002} & 0.019 & \textbf{12.1} & \textbf{0.734} & \textbf{0.013} & \textbf{0.111} \\
 & RUPTA & \textbf{1.000} & \textbf{0.002} & \textbf{0.013} & 24.2 & 0.725 & 0.053 & 0.114 \\
 & Check123 & 0.982 & 0.065 & 0.110 & 72.9 & 0.671 & 0.029 & 0.159 \\
\midrule
\multicolumn{9}{l}{\textit{Re-post on another channel}} \\
SDG ($\varepsilon=1$) & SDG-CI & \textbf{0.546} & \textbf{0.569} & \textbf{0.407} & \textbf{11.2} & 0.507 & 0.015 & 0.018 \\
 & MAPLE & 0.350 & 1.178 & 0.535 & 36.5 & \textbf{0.527} & \textbf{0.003} & \textbf{0.000} \\
 & Aug-PE & 0.027 & 10.557 & 0.814 & 45.1 & 0.522 & 0.084 & 0.035 \\
\cmidrule(l){2-9}
Anon. & AN-CI & \textbf{1.000} & \textbf{0.001} & 0.016 & \textbf{5.1} & \textbf{0.749} & \textbf{0.003} & \textbf{0.339} \\
 & RUPTA & \textbf{1.000} & 0.002 & \textbf{0.013} & 24.2 & 0.725 & 0.053 & 0.344 \\
 & Check123 & 0.982 & 0.065 & 0.110 & 72.9 & 0.671 & 0.029 & 0.358 \\
\midrule
\multicolumn{9}{l}{\textit{Advertisement Company}} \\
SDG ($\varepsilon=1$) & SDG-CI & \textbf{0.400} & \textbf{0.704} & \textbf{0.495} & \textbf{9.2} & \textbf{0.604} & 0.062 & 0.003 \\
 & MAPLE & 0.350 & 1.178 & 0.535 & 36.5 & 0.527 & \textbf{0.003} & 0.001 \\
 & Aug-PE & 0.027 & 10.557 & 0.814 & 45.1 & 0.522 & 0.084 & \textbf{0.000} \\
\cmidrule(l){2-9}
Anon. & AN-CI & \textbf{1.000} & 0.004 & 0.028 & \textbf{10.1} & \textbf{0.729} & 0.062 & \textbf{0.235} \\
 & RUPTA & \textbf{1.000} & \textbf{0.002} & \textbf{0.013} & 24.2 & 0.725 & 0.053 & 0.257 \\
 & Check123 & 0.982 & 0.065 & 0.110 & 72.9 & 0.671 & \textbf{0.029} & 0.282 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\small
\caption{Exact fidelity and privacy values behind Figure~\ref{fig:spider_datasets} (one audience per dataset). Raw values in natural units ($\uparrow$ higher is better, $\downarrow$ lower is better); best value per family and panel in bold (ties all bold). Len-W is the Wasserstein distance between text-length distributions. Leak is the attack success on the audience's private attributes: attribute-inference advantage over the majority baseline (clipped at 0, averaged over private attributes) for SDG, and LLM fuzzy reconstruction rate (averaged over private attributes) for anonymization. The figures plot MAUVE, $1/(1+\mathrm{KL})$, $1-\mathrm{TV}$, $1/(1+\text{Len-W}/100)$, Acc, $1-|\Delta|$ and $1-\text{Leak}$ on a fixed $[0,1]$ scale.}
\label{tab:spider_datasets}
\begin{tabular}{llrrrrr}
\toprule
 & Method & MAUVE$\uparrow$ & KL$\downarrow$ & TV$\downarrow$ & Len-W$\downarrow$ & Leak$\downarrow$ \\
\midrule
\multicolumn{7}{l}{\textit{Reddit}} \\
SDG ($\varepsilon=1$) & SDG-CI & \textbf{0.479} & \textbf{0.791} & \textbf{0.422} & \textbf{12.7} & 0.004 \\
 & MAPLE & 0.350 & 1.178 & 0.535 & 36.5 & \textbf{0.000} \\
 & Aug-PE & 0.027 & 10.557 & 0.814 & 45.1 & 0.001 \\
\cmidrule(l){2-7}
Anon. & AN-CI & \textbf{1.000} & \textbf{0.002} & 0.019 & \textbf{12.1} & \textbf{0.111} \\
 & RUPTA & \textbf{1.000} & \textbf{0.002} & \textbf{0.013} & 24.2 & 0.114 \\
 & Check123 & 0.982 & 0.065 & 0.110 & 72.9 & 0.159 \\
\midrule
\multicolumn{7}{l}{\textit{bioRxiv}} \\
SDG ($\varepsilon=1$) & SDG-CI & \textbf{0.420} & \textbf{1.750} & \textbf{0.463} & 72.2 & \textbf{0.000} \\
 & MAPLE & 0.097 & 3.217 & 0.689 & \textbf{55.0} & \textbf{0.000} \\
 & Aug-PE & 0.028 & 6.417 & 0.791 & 568.6 & 0.023 \\
\cmidrule(l){2-7}
Anon. & AN-CI & 0.999 & 0.019 & 0.077 & \textbf{10.8} & \textbf{0.360} \\
 & RUPTA & \textbf{1.000} & \textbf{0.011} & \textbf{0.037} & 11.0 & 0.380 \\
 & Check123 & 0.998 & 0.024 & 0.077 & 53.7 & 0.439 \\
\midrule
\multicolumn{7}{l}{\textit{Zillow (Internal Audit)}} \\
SDG ($\varepsilon=1$) & SDG-CI & \textbf{0.080} & 4.732 & \textbf{0.704} & \textbf{235.8} & 0.074 \\
 & MAPLE & 0.065 & \textbf{3.997} & 0.733 & 328.8 & \textbf{0.000} \\
 & Aug-PE & 0.010 & 10.928 & 0.926 & 1300.8 & 0.007 \\
\cmidrule(l){2-7}
Anon. & AN-CI & \textbf{0.959} & \textbf{0.115} & \textbf{0.160} & 31.0 & 0.400 \\
 & RUPTA & 0.698 & 0.668 & 0.269 & \textbf{26.3} & 0.395 \\
 & Check123 & 0.607 & 0.458 & 0.315 & 139.2 & \textbf{0.375} \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\small
\caption{Exact downstream accuracy and sex-gap values behind the Reddit panel of Figure~\ref{fig:spider_datasets}. Acc and $|\Delta|$ as in Table~\ref{tab:spider_audiences}; best value per family in bold.}
\label{tab:spider_datasets_reddit_fair}
\begin{tabular}{llrr}
\toprule
 & Method & Acc$\uparrow$ & $|\Delta|\downarrow$ \\
\midrule
\multicolumn{4}{l}{\textit{Reddit}} \\
SDG ($\varepsilon=1$) & SDG-CI & \textbf{0.546} & 0.038 \\
 & MAPLE & 0.527 & \textbf{0.003} \\
 & Aug-PE & 0.522 & 0.084 \\
\cmidrule(l){2-4}
Anon. & AN-CI & \textbf{0.725} & \textbf{0.034} \\
 & RUPTA & \textbf{0.725} & \textbf{0.034} \\
 & Check123 & 0.681 & 0.050 \\
\bottomrule
\end{tabular}
\end{table*}

==> proof_v0.tex <==
% Appendix: proof of Feature-DP for SDG-CI. Use with \input{proof_v0}
\section{Proof of Feature Differential Privacy}
\label{app:dp_proof}

A record is $z=(t,x)$ with $x=\Ext(t)$ or, on Reddit and bioRxiv, the attributes shipped with the data, and its disclosed part under context $c_j$ is $\Psi_j(z)=x[\Apub(c_j)]$. Everything else about $z$, including the text $t$, is protected. We assume that (A1) the schema $\mathcal S$, the coarsening maps, and $\Ext$ are fixed independently of $D$; (A2) the partition depends only on $\mathcal S$ and $c_j$; (A3) the LLM calls in Algorithm~\ref{alg:sdg_ci} see only rows of $\widehat T$ (real public values and synthetic private values), earlier candidates, and in-context examples from a held-out split disjoint from $D$, which are treated as public, never private text; and (A4) the guarantee concerns coarsened attribute values, and mapping a coarsened value back to a schema value (App.~\ref{app:coarsening}) draws uniformly from the public value list, which is post-processing. We treat corpora and outputs as multisets.

Both stages of \sdgci{} are accounted in zCDP~\cite{bun2016concentrated}, so we use the zCDP form of Feature-DP, where $\mathrm{D}_\alpha$ denotes the R\'enyi divergence of order $\alpha$.

\begin{definition}[Feature-zCDP]
\label{def:fzcdp}
A mechanism $\mathcal M$ is $\rho$-feature-zCDP relative to $\Psi_j$ if there is a simulator $\mathrm{sim}$ such that for every corpus $D$, record $z$, and $\alpha>1$, with $Y=\mathcal M(D\cup\{z\})$ and $Z=\mathrm{sim}(D,\Psi_j(z))$, we have $\mathrm{D}_\alpha(Y\|Z)\le\rho\alpha$ and $\mathrm{D}_\alpha(Z\|Y)\le\rho\alpha$.
\end{definition}

The usual conversion from zCDP to $(\varepsilon,\delta)$-DP, e.g., $\varepsilon=\rho+2\sqrt{\rho\ln(1/\delta)}$~\cite[Prop.~1.3]{bun2016concentrated}, uses only these two divergence bounds. Applied to $(Y,Z)$ and $(Z,Y)$, it shows that $\rho$-feature-zCDP implies $(\varepsilon,\delta)$-Feature-DP for every $\delta\in(0,1)$.

\begin{theorem}
\label{thm:e2e}\label{thm:aim}
\sdgci{} (Algorithm~\ref{alg:sdg_ci}) with $\rho=\rho_{\mathrm{AIM}}+\rho_{\mathrm{PE}}$ is $\rho$-feature-zCDP relative to $\Psi_j$, and hence $(\varepsilon,\delta)$-Feature-DP for the conversion of $\rho$. Conditional AIM (Algorithm~\ref{alg:cond_aim}) alone is $\rho_{\mathrm{AIM}}$-feature-zCDP.
\end{theorem}

\begin{proof}
\sdgci{} uses the private corpus in only two ways. It copies each record's public attributes (Algorithm~\ref{alg:cond_aim}, line~\ref{line:copy}), and it releases a sequence of noisy measurements $m_1,\ldots,m_M$: the one-way marginals of $\Apriv(c_j)$ (line~\ref{line:oneway}), the exponential-mechanism selections and Gaussian marginals of the AIM loop (lines~\ref{line:select}--\ref{line:measure}), and the $T_{\mathrm{PE}}+1$ noisy vote histograms of PE (Algorithm~\ref{alg:sdg_ci}, line~\ref{line:noise}). Each measurement may depend adaptively on earlier ones and on the outputs of the steps below. All other steps, namely merging, Private-PGM, sampling, expanding merged values, and LLM generation and selection, are a fixed randomized function $G$ of these inputs, by (A3). Hence $\mathcal M(D)=G(P(D),m_1(D),\ldots,m_M(D))$, where $P(D)$ is the multiset of public rows $\Psi_j(z')$, $z'\in D$.

The simulator runs the same algorithm but computes every measurement on $D$ instead of $D\cup\{z\}$: $\mathrm{sim}(D,\Psi_j(z))=G(P(D)\cup\{\Psi_j(z)\},m_1(D),\ldots,m_M(D))$. Parameters that depend on the record count, such as $\delta=1/n$, are set from $|D|+1$. It never uses $x[\Apriv(c_j)]$ or $t$. Since $P(D\cup\{z\})=P(D)\cup\{\Psi_j(z)\}$, the outputs $Y$ and $Z$ differ only in whether the measurements are computed on $D\cup\{z\}$ or on $D$.

Adding $z$ changes each measurement by a bounded amount, given the same history. Every marginal in the workload contains a private attribute (line~\ref{line:workload}), and $z$ falls into exactly one of its cells, so its $\ell_2$ sensitivity is $1$. The vote histograms also change by at most one in $\ell_2$ norm, since $z$ casts one vote (or, with soft voting, weights summing to one) using its text $t$. The selection score changes by at most $w_r$, since $\hat p_{t-1}$, $\sigma_t$, and $n_r$ are fixed by the history, and the exponential mechanism is calibrated to $\max_r w_r$. A Gaussian measurement with noise $\sigma$ therefore bounds the RÃ©nyi divergence by $\alpha/(2\sigma^2)$, and a selection with parameter $\varepsilon_t$ by $\alpha\varepsilon_t^2/8$, in both directions~\cite{bun2016concentrated, mckenna_aim}.

By adaptive composition~\cite[Lemma~2.3]{bun2016concentrated}, the two measurement sequences are within $\rho\alpha$ of each other in both directions. Conditional AIM spends at most $0.1\rho_{\mathrm{AIM}}$ on the one-way marginals, and its loop spends exactly $0.9\rho_{\mathrm{AIM}}$, since line~\ref{line:final} shrinks the last round to the remainder. PE spends $\rho_{\mathrm{PE}}/(T_{\mathrm{PE}}+1)$ on each histogram through $\sigma_{\mathrm{PE}}=\sqrt{(T_{\mathrm{PE}}+1)/(2\rho_{\mathrm{PE}})}$. Applying the same $G$ to both sequences cannot increase the divergence, which gives the bound for $Y$ and $Z$ with $\rho$. Restricting to Conditional AIM and its outputs gives the bound with $\rho_{\mathrm{AIM}}$.
\end{proof}

Because $Z$ is produced without $t$ or $x[\Apriv(c_j)]$, the theorem bounds what the release reveals about the whole record beyond $\Psi_j(z)$, including content the schema does not capture. It does not limit inference from $\Psi_j(z)$ itself, which is released exactly, or membership inference (Limitations), and it does not apply to \anci{}, which has no formal guarantee.
